Entropies of tailored random graph ensembles: bipartite graphs, generalised degrees, and node neighbourhoods

We calculate explicit formulae for the Shannon entropies of several families of tailored random graph ensembles for which no such formulae were as yet available, in leading orders in the system size. These include bipartite graph ensembles with imposed (and possibly distinct) degree distributions for the two node sets, graph ensembles constrained by specified node neighbourhood distributions, and graph ensembles constrained by specified generalised degree distributions.

==> commands.tex <==
% general mathematical abbreviations

\newcommand{\is}{{\!=\!}}
\newcommand{\pprime}{{\prime\prime}}
\newcommand{\double}{{\prime\prime}}
\newcommand{\bra}{\langle}
\newcommand{\ket}{\rangle}
\newcommand{\bigbra}{\left\langle}
\newcommand{\bigket}{\right\rangle}
\newcommand{\order}{{\mathcal O}}
\newcommand{\smallo}{{\mathcal o}}
\newcommand{\sgn}{\textrm{sgn}}
\newcommand{\erf}{\textrm{erf}}
%\newcommand{\Tr}{\textrm{Tr}}
\newcommand{\id}{{\rm 1\!\!I}}
\newcommand{\one}{{\rm 1\!\!I}}
\newcommand{\openone}{{\rm 1\!\!I}}
\newcommand{\plus}{{\!+\!}}
\newcommand{\minus}{{\!-\!}}
\newcommand{\bnull}{{\mbox{\boldmath $0$}}}
\newcommand{\bd}{\begin{displaymath}}
\newcommand{\ed}{\end{displaymath}}
\newcommand{\vsp}{\vspace*{3mm}}
\newcommand{\room}{\rule[-0.1cm]{0cm}{0.6cm}}
\newcommand{\bigroom}{\rule[-0.4cm]{0cm}{1.0cm}}
\newcommand{\verybigroom}{\rule[-0.7cm]{0cm}{1.3cm}}
\newcommand{\extr}{{\rm extr}}

\newcommand{\F}{{\mathcal F}}
\newcommand{\R}{{\rm I\!R}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\real}{{\rm I\!R}}
\newcommand{\N}{{\rm I\!N}}
\newcommand{\B}{{\mathcal B}}
\newcommand{\D}{{\mathcal D}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\Z}{{\mathcal Z}}
\newcommand{\W}{{\mathcal W}}


% bold characters and symbols

\newcommand{\ba}{\ensuremath{\mathbf{a}}}
\newcommand{\bb}{\ensuremath{\mathbf{b}}}
\newcommand{\bc}{\ensuremath{\mathbf{c}}}
\newcommand{\bh}{\ensuremath{\mathbf{h}}}
\newcommand{\bk}{\ensuremath{\mathbf{k}}}
\newcommand{\bm}{\ensuremath{\mathbf{m}}}
\newcommand{\bq}{\ensuremath{\mathbf{q}}}
%\newcommand{\bs}{\ensuremath{\mathbf{s}}}
\newcommand{\bu}{\ensuremath{\mathbf{u}}}
\newcommand{\bv}{\ensuremath{\mathbf{v}}}
\newcommand{\bw}{\ensuremath{\mathbf{w}}}
\newcommand{\bx}{\ensuremath{\mathbf{x}}}
\newcommand{\by}{\ensuremath{\mathbf{y}}}
\newcommand{\bz}{\ensuremath{\mathbf{z}}}

\newcommand{\bA}{\ensuremath{\mathbf{A}}}
\newcommand{\bB}{\ensuremath{\mathbf{B}}}
\newcommand{\bC}{\ensuremath{\mathbf{C}}}
\newcommand{\bD}{\ensuremath{\mathbf{D}}}
\newcommand{\bE}{\ensuremath{\mathbf{E}}}
\newcommand{\bF}{\ensuremath{\mathbf{F}}}
\newcommand{\bG}{\ensuremath{\mathbf{G}}}
\newcommand{\bH}{\ensuremath{\mathbf{H}}}
\newcommand{\bI}{\ensuremath{\mathbf{I}}}
\newcommand{\bJ}{\ensuremath{\mathbf{J}}}
\newcommand{\bK}{\ensuremath{\mathbf{K}}}
\newcommand{\bL}{\ensuremath{\mathbf{L}}}
\newcommand{\bM}{\ensuremath{\mathbf{M}}}
\newcommand{\bN}{\ensuremath{\mathbf{N}}}
\newcommand{\bO}{\ensuremath{\mathbf{O}}}
\newcommand{\bP}{\ensuremath{\mathbf{P}}}
\newcommand{\bQ}{\ensuremath{\mathbf{Q}}}
\newcommand{\bR}{\ensuremath{\mathbf{R}}}
\newcommand{\bS}{\ensuremath{\mathbf{S}}}
\newcommand{\bT}{\ensuremath{\mathbf{T}}}
\newcommand{\bU}{\ensuremath{\mathbf{U}}}
\newcommand{\bV}{\ensuremath{\mathbf{V}}}
\newcommand{\bW}{\ensuremath{\mathbf{W}}}
\newcommand{\bX}{\ensuremath{\mathbf{X}}}
\newcommand{\bY}{\ensuremath{\mathbf{Y}}}
\newcommand{\bZ}{\ensuremath{\mathbf{Z}}}

\newcommand{\blambda}{{\mbox{\boldmath $\lambda$}}}
\newcommand{\bgamma}{{\mbox{\boldmath $\gamma$}}}
\newcommand{\balpha}{{\mbox{\boldmath $\alpha$}}}
\newcommand{\bbeta}{{\mbox{\boldmath $\beta$}}}
\newcommand{\bxi}{{\mbox{\boldmath $\xi$}}}
\newcommand{\bpsi}{{\mbox{\boldmath $\psi$}}}
\newcommand{\bphi}{{\mbox{\boldmath $\phi$}}}
\newcommand{\bomega}{{\mbox{\boldmath $\omega$}}}
\newcommand{\bsigma}{{\mbox{\boldmath $\sigma$}}}
\newcommand{\bl}{{\mbox{\boldmath $\ell$}}}
\newcommand{\btau}{{\mbox{\boldmath $\tau$}}}
\newcommand{\btheta}{{\mbox{\boldmath $\theta$}}}
\newcommand{\bEta}{{\mbox{\boldmath $\eta$}}}
\newcommand{\bLambda}{{\mbox{\boldmath $\Lambda$}}}
\newcommand{\bOmega}{{\mbox{\boldmath $\Omega$}}}

% hat characters and symbols

\newcommand{\hh}{\hat{h}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}

\newcommand{\hA}{\hat{A}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hQ}{\hat{Q}}

\newcommand{\hOmega}{\hat{\mbox{$\Omega$}}}

% bold and hat characters

\newcommand{\hbh}{\widehat{\mathbf{h}}}
\newcommand{\hbk}{\widehat{\mathbf{k}}}
\newcommand{\hbm}{\widehat{\mathbf{m}}}
\newcommand{\bhw}{\widehat{\mathbf{w}}}
\newcommand{\hbw}{\widehat{\mathbf{w}}}
\newcommand{\bhx}{\widehat{\mathbf{x}}}
\newcommand{\hbx}{\widehat{\mathbf{x}}}
\newcommand{\bhq}{\widehat{\mathbf{q}}}
\newcommand{\hbq}{\widehat{\mathbf{q}}}

\newcommand{\hbK}{\widehat{\mathbf{K}}}
\newcommand{\hbQ}{\widehat{\mathbf{Q}}}

% picture drawing

\newcommand{\wcirc}{\circle{30}}
\newcommand{\bcirc}{\circle*{31}}
\newcommand{\Size}{270}
\newcommand{\BSize}{200}
\newcommand{\here}{\makebox(0,0)}
\newcommand{\wbox}{{\circ}}
\newcommand{\bbox}{{\bullet}}
\newcommand{\whitesquare}{{\framebox(1.2,1.2){}}~}
\newcommand{\whitecircle}{{\large $\circ$}}
%\newcommand{\blacksquare}{\rule{1.3\unitlength}{1.3\unitlength}~}
\newcommand{\blackcircle}{{\large $\bullet$}}


% MG specific abbreviations

\newcommand{\rate}{\tilde{\eta}}
\newcommand{\s}{\sigma}
\newcommand{\si}{\sigma}
\newcommand{\del}{{\delta_{\!N}}}
\newcommand{\hbe}{\hat{\bf e}}
\newcommand{\notdelta}{\overline{\delta}}
\newcommand{\chiR}{\chi_{\!\!\!~_R}}
\newcommand{\freq}{f}

\newcommand{\TBF}{{\vspace*{3mm}\hrule\vspace*{1mm}
\begin{center}{TO BE FINISHED}\end{center}
\vspace*{1mm}\hrule\vspace*{3mm}}}

